Enhancing Malware Fingerprinting through Analysis of Evasive Techniques

As malware detection evolves, attackers adopt sophisticated evasion tactics. Traditional file-level fingerprinting, such as cryptographic and fuzzy hashes, is often overlooked as a target for evasion. Malware variants exploit minor binary modifications to bypass detection, as seen in Microsoft's discovery of GoldMax variations (2020-2021). However, no large-scale empirical studies have assessed the limitations of traditional fingerprinting methods on real-world malware samples or explored improvements. This paper fills this gap by addressing three key questions: (a) How prevalent are file variants in malware samples? Analyzing 4 million Windows Portable Executable (PE) files, 21 million sections, and 48 million resources, we find up to 80% deep structural similarities, including common APIs and executable sections. (b) What evasion techniques are used? We identify resilient fingerprints (clusters of malware variants with high similarity) validated via VirusTotal. Our analysis reveals non-functional mutations, such as altered section numbers, virtual sizes, and section names, as primary evasion tactics. We also classify two key section types: malicious sections (high entropy >5) and camouflage sections (entropy = 0). (c) How can fingerprinting be improved? We propose two novel approaches that enhance detection, improving identification rates from 20% (traditional methods) to over 50% using our refined fingerprinting techniques. Our findings highlight the limitations of existing methods and propose new strategies to strengthen malware fingerprinting against evolving threats.

==> arxive_esorics/sections/0_abstract.tex <==
\begin{abstract}

As malware detection methods become more advanced and widespread, malware authors are responding by adopting more sophisticated evasion mechanisms. However, traditional methods based on file-level fingerprinting, including cryptographic and fuzzy hashes, are often overlooked as a potential target for evasion. In practice, malware attacks frequently employ minor variations within binary components to bypass conventional fingerprinting techniques, as evidenced by Microsoft's identification of the GoldMax variations in 2020 and 2021.
Despite this, there have not been any extensive empirical studies that delve into the limitations of traditional malware fingerprinting techniques when used on real-world samples, or how their performance could be enhanced.

This paper addresses the gaps in understanding file variants in malware by answering three key questions: 
(1) To what extent are file variants used in malware samples? We conduct an empirical study of 4 million Windows Portable Executable (PE) files, 21 million sections, and 48 million resources, divided into four groups over time to validate our analysis. Our findings suggest a significant degree of similarity (70-80\%) in deeper segments of PE files, including similar APIs in Import Libraries and common executable sections.
(2) What evasive techniques involving file variants can be identified? We identify clusters of files with high similarities in Import Libraries and common executable sections, labeled  these clusters \textit{``Resilient fingerprints''} after validating their maliciousness. Our qualitative analysis across four dataset groups reveals non-functional mutations as primary evasive variant tactics, along with two types of executable sections: malicious (high entropy $>$ 5) and camouflage (entropy = 0).
(3) How can these characteristics improve malware fingerprinting? We propose two novel approaches, \textit{top-down} and \textit{bottom-up}, leveraging insights from the previous questions. These approaches enhance malware fingerprinting and enable the identification of resilient fingerprints. Using a dataset of 4 million feeds from VirusTotal, we demonstrate a potential improvement in fingerprinting, with over 50\% of malware identified compared to 20\% using traditional approaches.

%no large-scale empirical studies have investigated the limitations of traditional malware fingerprinting methods applied to actual samples obtained from the wild, and how their effectiveness might be improved.

%This paper addresses these gaps by answering three key questions: (1) To what extent are file variants commonly used in malware samples? To answer this question, we conduct an empirical study of a large-scale dataset of 4 million Windows Portable Executable (PE) files' reports, 21 million sections, and 48 million resources, which we divide into four chronological groups to validate our analysis. Our findings suggest a significant degree of similarity, ranging from 70\% to 80\%, in the deeper segments of PE files, including similar APIs in Import Libraries and common executable sections. (2) What types of evasive techniques involving file variants can be identified? To address this, we group files that exhibit high similarities in their Import Libraries and common executable sections and labelled these clusters \textit{``Resilient fingerprints''} after validating their maliciousness ground truth through the Virustotal vendor labels. We then carry out a qualitative analysis across our dataset composed of four groups to identify the variant parts of the resilient fingerprints. Our findings reveal that non-functional mutations - such as alterations in the number of sections, virtual size, virtual address, and section names - are widely employed as primary evasive variant tactics. We also identify two executable sections of interest that are similar within each resilient fingerprint, which we refer to as malicious sections (high entropy > 5) and camouflage sections (entropy = 0). (3) How can we use these identified characteristics to improve malware fingerprinting? To answer this question, we propose two novel approaches named top-down and bottom-up leveraging the insights obtained from answering the previous two questions. They enhance malware fingerprinting and enable the identification of resilient fingerprints. Using a large dataset of 4 million feeds from VirusTotal, our findings indicate a large potential improvement in fingerprinting, with more than 50\% of malware being identified compared to 20\% using traditional fingerprinting approaches.



\end{abstract}

% The Top-Down approach clusters these resilient fingerprints based on similarities in Import Libraries before diving deeper into the malicious and camouflage sections, whereas the Bottom-Up approach first uses the invariant parts within the identified malicious and camouflage sections and then goes up to group files.

==> arxive_esorics/sections/1_introduction.tex <==
\section{Introduction}

%Static and dynamic malware analysis have advanced malware detection and prevention.


Advancements in malware detection and prevention have been made possible through static and dynamic malware analysis. Static analysis (e.g., ~\cite{anderson2018ember,downing2021deepreflect}), examines file attributes without executing the file, while dynamic analysis (e.g., ~\cite{kuchler2021does,kilgallon2017improving}) monitors the behavior of the software when it is run in a virtual environment.
Although static analysis is faster than dynamic analysis, it can become time-consuming when dealing with large datasets and extracting all pertinent file characteristics, including disassembly using commercial tools such as IDA Pro~\cite{IDAPro}.

%Static analysis is faster than dynamic analysis. However, when dealing with large datasets, extracting all relevant file characteristics, including obtaining disassembly using commercial tools like IDA Pro~\cite{IDAPro}, can still be time-consuming. 


As a result,  malware fingerprinting is often used as an initial screening (or {\it triaging}) method~\cite{sikorski2012practical} to reduce the scope of further investigation. Malware fingerprinting relies primarily on file hashing, generating checksums or unique identifiers for initial triaging. Cryptographic hashing and fuzzy hashing are the two prevalent techniques for hash-based file-level fingerprinting~\cite{oliver2021designing}. The SHA-256 cryptographic hash, in particular,  is commonly used to query databases such as VirusTotal~\cite{virustotal} to determine a file's maliciousness. Hashes serve as labels shared among security analysts to identify and query malware in online repositories.

% Advances in static and dynamic malware analysis have significantly improved the ability to detect and prevent malware attacks. Static analysis techniques~\cite{anderson2018ember,downing2021deepreflect} involve examining the characteristics of a file without executing it, whereas dynamic analysis techniques observe the behavior of the software as it runs in a virtual environment~\cite{mariconti2016mamadroid,jindal2019neurlux,wang2020you}.  Static analysis is notably faster than dynamic analysis. However, when dealing with large datasets, the process of extracting all relevant file characteristics, including obtaining disassembly using commercial tools like IDA Pro~\cite{IDAPro}, can still be time-consuming. As a result, malware fingerprinting is often used for detection as the first {\it triaging} mechanism~\cite{sikorski2012practical} to narrow the search space of files for further investigation. 

%Static analysis offers notable advantages in terms of speed compared to dynamic analysis. 



% Malware fingerprinting is primarily based on file hashing. The output of hashing, which is commonly used and shared between cybersecurity teams, takes the form of checksums or unique identifiers for first triaging. There are two types of hash-based file-level fingerprinting techniques: cryptographic hashing and fuzzy hashing~\cite{oliver2021designing}. It is common practice to use the SHA-256 cryptographic hash to query a knowledge database like VirusTotal~\cite{virustotal} to determine whether a file is malicious or not. Security analysts use hashes as labels, which are shared with other analysts to help them identify malware. They are subsequently queried in online repositories to determine if the hash has been previously identified. 


File-level hash fingerprinting is fast but faces challenges in identifying similar malware due to traditional cryptographic hashing. Cryptographic hashing conceals the correlation between the original entity and the hash value, resulting in radically different hashes even with minor changes in the original file. Fuzzy hashing overcomes this limitation by producing similar hashes for slightly changed files, making it more tolerant to evasion methods~\cite{oliver2013tlsh}. For example, Microsoft 365 confirmed that the GoldMax malware sample, submitted to VirusTotal in September 2020 and reappeared in June 2021 with a new hash~\cite{goldmaxMS}, was identified as the same by fuzzy hashing, which cryptographic hashing failed to do.

% While file-level hash fingerprinting is fast and useful, traditional cryptographic hashing poses a challenge in identifying similar malware. This is because cryptographic hashing  relies on concealing the correlation between the original entity and the hash value. Even one character change in the original entity, such as a file, results in a radically different hash, making identifying similar malware challenging. Another type of malware fingerprinting is fuzzy hashing. This overcomes the limitations of cryptographic hashing by producing similar hashes even when files are slightly changed, thereby making it more tolerant to evasion methods~\cite{tlsh}. Microsoft 365 recently confirmed that the GoldMax malware sample was first submitted to VirusTotal in September 2020, then reappeared in June 2021 with a new hash~\cite{goldmaxMS}. Despite some variation, both versions of GoldMax were captured by fuzzy hashing as the same, which cryptographic hashing failed to do. 


Security analysts, including Microsoft Threat Intelligence Center, have observed indications (e.g., GoldMax malware) that attackers exploit limitations in both types of hashes by creating multiple copies of sophisticated malware with variations, resulting in significantly different new ones~\cite{goldmaxMS}. Despite numerous studies on various malware-related activities, such as living off the land~\cite{barr2021survivalism}, IoT~\cite{alrawi2021circle}, Linux~\cite{cozzi2018understanding}, and sandboxing~\cite{yong2021inside}, \textit{there has been no systematic large-scale empirical study investigating malware fingerprinting from real samples in the wild}. Conducting such a study would address the important question of whether a large number of functionally similar malware goes undetected by traditional fingerprinting methods? Strengthening the malware fingerprinting stage is crucial for early triaging, enhancing the explainability and effectiveness of subsequent, more extensive, and expensive analysis forms. This motivates our study, which addresses the following three research questions (RQs):

%Security analysts, including Microsoft Threat Intelligence Center, have reported  indications (e.g., GoldMax malware) that attackers have exploited the limitations of both types of hashes by creating multiple copies of sophisticated malware with variations resulting in significantly different new ones~\cite{goldmaxMS}. However, while there have been many studies investigating various malware-related activities, such as living off the land~\cite{barr2021survivalism}, IoT~\cite{alrawi2021circle}, Linux~\cite{cozzi2018understanding}, and sandboxing~\cite{yong2021inside}, there has been no systematic large-scale empirical study investigating malware fingerprinting from real samples in the wild. Conducting such a study would answer the important question: Is there a large number of functionally similar malware being undetected by traditional fingerprinting methods? Strengthening the malware fingerprinting stage is crucial for the early triaging of potentially a large number of files, as it can enhance the explainability and effectiveness of subsequent, more extensive, and expensive forms of analysis. This motivates our study, which we address through the following three research questions (RQs):\\

{\bf RQ1.} To what extent are file variations commonly used in malware samples?

Building on this, we shed light on some of the trends in the current threat landscape to identify:

{\bf RQ2.}	What file variation evasive methods can be identified in each malware sample?

{\bf RQ3.}	How can we use the identified invariant file parts to improve malware fingerprinting? 


To study file variations within malware (RQ1), we systematically analyze high-level file information and detailed metadata to investigate their prevalence. Using our collected large-scale dataset from VirusTotal, containing reports for all worldwide files over two separate periods (9 months apart), we focus on PE files of Windows operating systems, constituting up to 50\% of all submissions. The dataset is divided into four chronological groups to assess the generalizability of our findings over time. Our analysis of deeper parts of the files, as depicted in Fig.~\ref{fig:VT_highlevel} reveals limited effectiveness of traditional fingerprinting techniques in detecting similar malware files: Cryptographic hashing identifies only 16-18.5\% of files, while fuzzy hashing detects 17.9-20.7\%. Deeper analysis shows that approximately 80\% of files share common Import Lists, 70\% have similar sections, and 80\% contain comparable resources (see Section~\ref{sec:prevelance}).

%To study to what extent file variations are used within malware (RQ1), we systematically analyse high-level file information and detailed metadata to investigate the prevalence of file variations. We collect a large-scale dataset from VirusTotal, which contains all reported files worldwide on a per-minute basis, over two separate periods of time (9 months apart), including detailed reports for each suspicious file at both high-level and detailed levels (see Section~\ref{sec:methodology} for further details). To ensure consistency in our analysis and findings, we focus on PE files of Windows operating systems, as they constitute up to 50\% all submitted files. We divide the dataset into four chronological groups to investigate the generalisability of our findings across different time periods. After examination, we found that traditional fingerprinting techniques have limited effectiveness in detecting similar malware files --- Cryptographic hash can only identify 16\% to 18.5\% of the files, while fuzzy hash performs slightly better, detecting 17.9\% to 20.7\% of the files. Analyzing deeper parts of the files as depicted in Fig.~\ref{fig:VT_highlevel} indicates a significant number of them shared common characteristics. Specifically, approximately 80\% of the files contained common Import Lists, while around 70\% of the files had some similar sections. Also, roughly 80\% of the files had comparable resources, as elaborated in Section~\ref{sec:prevelance}.


To address RQ2, we analyze files with common connections to investigate both variant and invariant components of malware samples. Firstly, we verify the malicious nature of these files using VirusTotal vendor labels. Secondly, we categorize files with variations but common critical invariant components as ``Resilient fingerprints'' and conduct a qualitative analysis. Our findings indicate that two invariant components within malware files, Import Libraries (containing a list of functionalities) and common sections (we refer to as ``camouflage sections'' and ``malicious sections''), can be used to detect a deep fingerprint. We observe that resilient fingerprints can be quite large (e.g., 27,091 files). Additionally, we identify non-functional variant evasive parts, such as the number of sections, virtual size, virtual address, and section names, which mutate between files to obfuscate the hash. These findings are detailed in Section~\ref{sec:malwarevariation}.

%To address RQ2, we delve deeper into the files with common connections and investigate both the variant and invariant components of the malware samples. Firstly, we establish the ground truth of these identified files and ensure their malicious nature using the VirusTotal vendor labels. Secondly, we categorize the files with variations (different traditional hash) but common critical invariant components into groups called \textit{``Resilient fingerprints''} and perform a qualitative analysis.  Our findings suggest that two invariant components within the malware files could be used to connect and detect a deep fingerprint together. These invariant components are the Import Libraries, which contain a list of functionalities and common sections --- we refer to as ``camouflage sections'' and ``malicious sections'', as explained in Section~\ref{sec:malwarevariation}. We find the size of these resilient fingerprints can be quite large (e.g., 27,091 files). On the other hand, we also identify many non-functional variant evasive parts that are mutated between these files to obfuscate the hash, including the number of sections, virtual size, virtual address, and section names (outlined in Section~\ref{sec:malwarevariation}).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/file_levels.pdf}
     % \vspace{0.2cm}
    \caption{VirusTotal report granularity per file.}
    \label{fig:VT_highlevel}
    \vspace{-6mm}
\end{figure}


To address RQ3, we aim to enhance malware fingerprinting by proposing two clustering approaches: Top-Down and Bottom-Up. The Top-Down approach initially clusters resilient fingerprints based on similarities in Import Libraries and functionalities, then identifies common camouflage and malicious sections within each cluster. In contrast, the Bottom-Up approach clusters files based on common sections like camouflage and malicious sections. Our methods consistently perform well across four datasets, with both approaches successfully identifying between 30\% (Top-Down) and 58\% (Bottom-Up) of reported suspicious files using resilient fingerprinting strategies, outperforming traditional mechanisms by up to three times. Our work aims to complement existing fingerprinting techniques rather than replace them entirely, enhancing early triaging efforts with a more comprehensive mechanism capable of capturing a broader spectrum of variations in common malware files. Further details can be found in Section~\ref{sec:detectionimprovment}.

%To address RQ3, we aim to enhance malware fingerprinting by leveraging the findings from the previous two RQs. We propose two clustering approaches, Top-Down and Bottom-Up. As depicted in VirusTotal detailed level in Figure~\ref{fig:VT_highlevel}, the Top-Down approach initially clusters resilient fingerprints based on similarities in their Import Libraries and a list of functionalities. It then proceeds to identify common camouflage and malicious sections within that cluster. On the other hand, the Bottom-Up approach clusters all files from lower levels relying on common sections, such as camouflage and malicious sections. Our proposed methods have demonstrated consistent performance across four datasets. Both approaches have successfully identified between 30\% (Top-Down) and 58\% (Bottom-Up) of reported suspicious files connected using resilient fingerprinting strategies, outperforming traditional fingerprinting mechanisms by up to three times. Our work is intended to augment the existing traditional fingerprinting techniques, rather than replace them altogether. Our proposed approaches are not to classify files as malicious or benign but rather  have been designed to enhance early triaging efforts by implementing a more comprehensive and thorough fingerprinting mechanism. This mechanism can capture a broader spectrum of variations of common malware files, as detailed in Section~\ref{sec:detectionimprovment}.


By answering the three RQs, this paper makes the following main contributions:

\begin{itemize}
    \item To the best of our knowledge, this paper presents the first large-scale systematic analysis of malware file variations and quantifies the limitations of traditional file-level fingerprinting.
    
    \item We systematically identify file variation evasive methods for bypassing traditional fingerprinting and significant invariant components that can enhance early triage fingerprinting.
    
    \item We propose two novel approaches, Top-Down and Bottom-Up, for identifying similar files at different levels, improving the efficacy of the early triage process.

    \item Our evaluation is extensive, based on a dataset from VirusTotal containing over 4 million file reports, 21 million sections, and 48 million resources. Results show high prevalence of similarities in low-level parts, while traditional hash-based methods achieve only 20\% detection rate within the 4 million feeds. Using the identified invariant parts, the paper demonstrates a more than 50\% improvement in early triage fingerprinting compared to traditional methods. Additionally, we plan to make our code and analysis public for future research and practice in the field.
\end{itemize}



==> arxive_esorics/sections/2_background_related.tex <==
\section{Background}\label{sec:background}

\subheading{VirusTotal Platform.}
VirusTotal is a widely known service that scans files and web addresses to detect whether they are malicious~\cite{virustotal}. With file scanning as a primary feature, it collaborates with 71 external security providers (see the full list at~\cite{virustotal}). When a file is submitted via the scanning API, VirusTotal performs two actions:  (1) searches for an already existing file hash (SHA256) within their cached database, if the hash does not exist, then (2) forwards the file to these vendors (i.e., anti-virus engines or online scanning services). 
VirusTotal retains records of the scanned files and corresponding results obtained from vendors in its database, which can be queried via the VirusTotal Report API.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.6\linewidth]{figures/Virustotal.pdf}
%      % \vspace{0.2cm}
%     \caption{VirusTotal Feeds APIs and interaction with third-party security vendors overview.}
%     \label{fig:Virutotal}
%     %\vspace{-8mm}
% \end{figure}

\subheading{Malware Fingerprinting and Vendor Labeling.}\label{sec:malware:labels}
The research community extensively uses VirusTotal to identify malicious files~\cite{invernizzi2014nazca,kolodenker2017paybreak,kotzias2016measuring,sharif2018predicting,sarabi2018characterizing,schwartz2018using,thomas2016investigating,wong2018tackling}, as well as suspicious IP addresses and URLs~\cite{wang2014whowas,tian2018needle}. Researchers often integrate labels from multiple vendors due to disagreements, with VirusTotal returning 71 labels from vendors for each file. Most papers use a threshold $t$ to consider a file malicious if at least $t$ vendors label it as such, with $t$ typically set to 2 to 4~\cite{invernizzi2014nazca,kolodenker2017paybreak,kotzias2016measuring,sharif2018predicting,wang2014whowas}, and occasionally relaxed to 1~\cite{sarabi2018characterizing,schwartz2018using,thomas2016investigating,tian2018needle,wong2018tackling}. Rarely have larger thresholds such as 40 been used but be ineffective~\cite{cai2016inferring,korczynski2017capturing,zhu2020measuring}. This study uses a conservative $t$=4, following the majority of literature, to determine the ground truth of collected samples.

%The research community has extensively used VirusTotal to identify malicious files~\cite{invernizzi2014nazca,kolodenker2017paybreak,kotzias2016measuring,sharif2018predicting,sarabi2018characterizing,schwartz2018using,thomas2016investigating,wong2018tackling} as well as suspicious IP addresses and URLs~\cite{wang2014whowas,tian2018needle,wwwchain19,zhao2019decade}. Researchers usually integrate the labels from several vendors because vendors frequently disagree with one another as they are using different mechanisms to check those files. Remember that when a file is provided, VirusTotal returns 71 labels from the vendors. We find that the majority of papers specify a threshold $t$: the file is considered malicious if at least $t$ vendors return a ``malicious'' label. The majority of papers set $t$ = 2 to 4~\cite{invernizzi2014nazca,kolodenker2017paybreak,kotzias2016measuring,sharif2018predicting,wang2014whowas}, while a few papers further relax $t$ = 1~\cite{sarabi2018characterizing,schwartz2018using,thomas2016investigating,tian2018needle,wong2018tackling}. On the other hand, rarely researchers use a large threshold such as 40 when labelling malware files~\cite{cai2016inferring,korczynski2017capturing}, which has been shown to be ineffective~\cite{zhu2020measuring}. We therefore use a conservative $t$=4 following the majority of literature when deciding the ground truth of the collected samples.

%\subsection{Existing studies.} \sharif{We talk here about few measurement studies.}
%\subsection{Motivational Scenario}\label{sec:malware:labels}

==> arxive_esorics/sections/3_methodology.tex <==
\section{Methodology}\label{sec:methodology}
We conduct a systematic large-scale empirical study on real-world malware samples to analyze their evasive strategies. This section outlines our approach to data collection, data characteristics, and the systematic investigation of our research questions.\\

\subheading{Data Collection.} We use the VirusTotal API, specifically the File Feeds~\cite{virustotal}, to access detailed reports on files worldwide. These reports are JSON-encoded structures arranged in batches generated every minute, containing information about the file's header, import list functions, sections, and resources (see Figure~\ref{fig:VT_highlevel}). We collect these reports automatically using a scheduled {\it cron} job. To ensure the validity and generalizability of our findings, we gather VirusTotal batches from two distinct time periods: a ten-week period from March 29th, 2022, to June 25th, 2022, and a three-week period from March 27th, 2023, to April 17th, 2023.


\subheading{Data Characteristics.} (1) \textit{File Types:} We analyze the file types in the collected batches using the ``FileType'' tag within each report, defined by the VirusTotal community. The top ten most common file types are Win32 EXE, HTML, Win32 DLL, Win64 EXE, XML, ZIP, TXT, Win64 DLL, ELF executable, and PDF. About half of the files are PE files from Windows operating systems, consistent with previous findings~\cite{song2016learning}. PE files, including Win32 EXE, Win32 DLL, Win64 EXE, and Win64 DLL, are selected for studying file variations due to their abundance and suitability for reliable empirical study.
(2) \textit{PE File Report Structure:} The report structure for a file can be categorized into high level and detailed level. The high level includes metadata like submission date/time, type, hash (MD5, SHA256, and TLSH), size, and vendors' votes on the file's maliciousness. The detailed part focuses on deeper file segments, including import libraries, list functionalities, code block sections, and resources like icons. VirusTotal provides detailed metadata for each of these, such as the number of sections or imports, along with characteristics like content hash, entropy, name, virtual size, and virtual address.





% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/VTreport_structure.png}
%      % \vspace{0.2cm}
%     \caption{VirusTotal report granularity -- detailed level.}
%     \label{fig:VT_lowlevel}
%     %\vspace{-8mm}
% \end{figure}

\subheading{Systematic Process.} To ensure study reliability, we divide the collected data from March to June 2022 into three groups (1-3), and the second dataset from March to April 2023 into the fourth group. Each group contains slightly over three weeks of file reports, with approximately 1,061,151 reports per group (Table~\ref{tb:group_details}). A relationship is observed between files and their number of sections and resources. On average, files have around 5 sections and 12 resources, with most having 3 sections and a smaller portion having more than 9 sections. Additionally, Table~\ref{tb:filetype} in the Appendix \ref{appendix:vt_filedistribution} presents the distribution of file types. The majority of files (around 60\%) are Win32 EXE, followed by Win32 DLL files (approximately 19\%). The combined percentage of Win64 EXE/DLL files is less than 20\%. Notably, a significant portion of the files (between 34\% and 42\%) are categorized as benign by VirusTotal vendor labeling. Table~\ref{tb:benignLabels} in the Appendix \ref{appendix:vt_filedistribution} shows detailed label statistics.

%To ensure study reliability, we divide the collected data from March to June 2022 into three groups (1-3), and the second dataset from March to April 2023 into the fourth group. Each group contains slightly over three weeks of file reports, with approximately 1,061,151 reports per group (Table~\ref{tb:group_details}). A relationship is observed between files and their number of sections and resources. On average, files have around 5 sections and 12 resources, with most having 3 sections and a smaller portion having a larger number of sections ($>$9). Additionally, Table~\ref{tb:filetype} presents the file types distribution. The majority of the files (around 60\%) are Win32 EXE, followed by Win32 DLL files (approximately 19\%). The combined percentage of Win64 EXE/DLL files is less than 20\%. Notably, a significant portion of the files (between 34\% and 42\%) are categorized as benign by VirusTotal vendor labeling. Table~\ref{tb:benignLabels}  shows detailed label statistics.

% To ensure the reliability of our study, we partition the collected data from March to June 2022, into three groups (1-3), and the second dataset from March to April 2023, into the fourth group. Each of which contains just above three weeks of file reports. Our aim from this step is to examine whether the obtained insights from one group could be confirmed from other groups collected in slightly different timeframes. As shown in Table~\ref{tb:group_details}, we select the same number of reports per group, around $1,061,151$. It is clear that there is a notable relationship between the files and their number of sections and contained resources. On average, every file has around 5 sections and 12 resources. It is worth mentioning that on deeper analysis, we find that most files have 3 sections and the rest might have a large number of sections $>9$. On the other hand, a large number of the collected files have $<10$ resources. In Table~\ref{tb:filetype}, we present the estimated distribution of file types across four of these groups. 
% The majority, accounting for approximately 60\%, consist of Win32 EXE files, followed by Win32 DLL files at around 19\%. The combined percentage of Win64 EXE/DLL files is less than 20\%. In terms of VirusTotal vendor labeling, it is important to note that a considerable portion of the files fall into the benign category. Specifically, between 34\% and 42\% of these files are categorized as having low maliciousness, and thus, we classify them as benign (refer to Table~\ref{tb:benignLabels} in Appendix~\ref{appendix:VTlabelling} for detailed label statistics).


%Win32 EXE constitutes the largest proportion at approximately 60\%, followed by Win32 DLL at around 19\%. The combined percentage of Win64 EXE/DLL is less than 20\%. When it comes to VirusTotal vendor labeling, it's worth noting that a significant proportion of the files fall within the benign category. Specifically, around 34\% to 42\% of these files are deemed to have low maliciousness, and therefore, we consider them benign (See Table~\ref{tb:benignLabels} in Appendix~\ref{appendix:VTlabelling} for labels statistics).

\begin{table}[h]
\caption{Groups files, sections and resources detail.}
%\vspace{-0.1cm}
\centering
\resizebox{2.8in}{!}{
\begin{tabular}{l|r|r|r|r}
\hline
          & {\bf Group 1} & {\bf Group 2} & {\bf Group 3} & {\bf Group 4}\\ \hline
Files     & 1,061,151  & 1,061,151  & 1,061,151  & 1,061,151\\ \hline
Sections  & 5,679,597  & 5,481,258  & 5,441,488  & 6,263,307\\ \hline
Resources & 12,589,924 & 12,715,782 & 11,159,391 & 13,627,706\\ \hline
\end{tabular}}
\label{tb:group_details}
\end{table}




% \usepackage{multirow}

% \usepackage{multirow}




% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/groups.png}
%      % \vspace{0.2cm}
%     \caption{Group details.}
%     \label{fig:Virutotal}
%     %\vspace{-8mm}
% \end{figure}

==> arxive_esorics/sections/4_malware_prevalance.tex <==
\section{Prevalence of File Variation}\label{sec:prevelance}

This section addresses RQ 1: \textit{To what extent are file variations commonly used in malware samples?} Our goal is to explore file similarities beyond traditional fingerprinting. Here, we provide an overview, examine different file components for potential similarities with examples, and present our results and their consistency across the four groups.\\

\subheading{Overview.} We start by examining how many similar files can be identified using traditional file fingerprinting techniques. We take SHA256 and TLSH to represent cryptographic and fuzzy hashing respectively. 
The obtained results seem consistent across the 4 groups with low similarities of 16\%-20\% (see Results Section~\ref{sec:results}). We then investigate the prevalence of non-functional file variations, which are done to alter the hash of the file. This is an evasion technique employed by malware authors to bypass traditional hash-based fingerprinting. For example, a malware author may modify a previously detected malicious file by padding the file with non-functional content, thereby changing the hash and avoiding detection. We identify three parts within a file that are representative of the actual intent of the file. When these are common between two files with unique hashes, this is indicative of file variations. These parts are the import libraries' list of functionalities, sections, and resources. Next, we elaborate further on each of these parts with illustrations before presenting the obtained results.

\subheading{Import Libraries with List of Functions.}\label{sec:importList}
The import list includes functions imported from other libraries that files use to achieve their purpose. For example, in Figure~\ref{fig:importlist}, a sample malware file imports functions from six libraries, providing insights into its intentions. For instance, it imports from \textit{ADVAPI32.DLL}, which grants access to Windows components like the Service Manager and Registry. Functions 4-7 indicate the file's action of altering the Registry by creating an entry and setting its value. Another example is the import from \textit{KERNEL32.DLL}, which offers core functionalities like file access and manipulation. Functions 2-7 show the file's actions of copying files, creating processes, and deleting those files.
Similarities in import lists are reliable indicators of common intent. However, we adopt a cautious approach by stipulating that for us to consider two files as variations, they must exhibit a 100\% similarity of the entire imported list of libraries and imported functions while having different file hashes. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/ImportList.pdf}
     % \vspace{0.2cm}
    \caption{Import List -- each pair of boxes shows the imported library and its list of functions.}
    \label{fig:importlist}
    %\vspace{-8mm}
\end{figure}

%\subsection{Header}

\subheading{Sections of PE Files - Executable Code.}
A PE file contains sections with executable code or relevant details. These sections, such as \textit{``.text''}, \textit{``.rdata''}, \textit{``.data''}, and \textit{``.rsrc''}, serve different purposes like storing executable code, read-only data, global data, and resources respectively. Identifying two files with the same code blocks but different hashes can indicate malware variation. Therefore, we use sections as another indicator of file variations. Our detailed VirusTotal feeds provide section-level information, including content hash, name/type, entropy, raw\_size, virtual\_address, and virtual\_size, which could be reliable for identifying similarities.

% A PE file comprises several sections, each containing executable code or relevant details related to the executable code. The sections could be one of the following types: \textit{``.text''}  contains the executable code; \textit{``.rdata''} holds read-only data that is globally accessible within the program; \textit{``.data''} stores global data accessed throughout the program; \textit{``.rsrc''} stores resources needed by the executable.

% Having two files sharing the same code blocks while producing two different file hashes might be an indication of malware file variation. Consequently, we use sections as another indication of the prevalence of file variations. Through the collected VirusTotal feeds, we have detailed information about every section within the file. For example, Table~\ref{fig:sectionData} shows one of four sections of a real malware sample we collected. The table shows that the sections' metadata has fine-grained details, including its content hash, name/type, entropy, raw\_size, virtual\_address, and virtual\_size, which could be a reliable source to identify the similarities.\\  

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.90\linewidth]{figures/section.png}
%      % \vspace{0.2cm}
%     \caption{Section metadata.}
%     \label{fig:sectionData}
%     %\vspace{-8mm}
% \end{figure}

% \begin{table}
% \centering
% \caption{Section metadata provided by VirusTotal.}
% %\vspace{-0.3cm}
% \centering
% \label{fig:sectionData}
% \resizebox{2.4in}{!}{
% \begin{tabular}{r|l} 
% \hline
% {\bf Metadata}         & {\bf Value}                             \\ 
% \hline
% MD5              & a0a2aedaaf49ad428951a94bf6038890  \\ 
% \hline
% Chi-squared      & 80,784.76                          \\ 
% \hline
% Entropy          & 7.5                               \\ 
% \hline
% Name             & updateRegistry.text                             \\ 
% \hline
% Raw\_size        & 32,340                             \\ 
% \hline
% Virtual\_Address & 4,096                              \\ 
% \hline
% Virtual\_Size    & 32,340                             \\ 
% \hline
% Flags    & {\tt rwx}                             \\ 
% \hline
% \end{tabular}}
% \vspace{-3mm}
% \end{table}
\subheading{Resources of PE Files -- non-Executables.}
The resources part of a file contains non-executable materials such as icons, images and strings. Resource types could include Data, ASCII text, Image/x-png, Lotus 1-2-3, Image/gif, or Audio/mpeg. Our findings suggest that resources may be less effective in indicating the intent of a file as they can be similar between behaviorally different files. This is because these resources, such as Microsoft logos, may be used by both benign and malware samples. %(refer to Appendix~\ref{sec:resourcesUnrialiable} for further detail). 
Similar to sections, the available resource's metadata from VirusTotal feeds has detailed information, including its content hash, type, entropy, chi2, and typeX.  

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.90\linewidth]{figures/section.png}
%      % \vspace{0.2cm}
%     \caption{Resources metadata.\sharif{Figure need to be changed to resources}}
%     \label{fig:resourcesData}
%     %\vspace{-8mm}
% \end{figure}

\subsubsection{Results.}\label{sec:results}
We group files together based on content similarity using three critical file parts and compare this approach to traditional file-level hash fingerprinting. Figure~\ref{fig:fileprevalnce} illustrates the results across the four groups. To calculate redundancy on the y-axis, we apply a unique function to a set of $N$ file hashes (e.g., 100) to determine the count of unique hashes, represented as $U$ (e.g., 84). The number of redundant hashes is then found by subtracting $U$ from $N$, resulting in 16. Traditional file-level hash (SHA256 and TLSH) identifies only 16\%-20\% file redundancy within each group. However, deeper analysis using critical file parts like the import list, sections, and resources reveals higher similarities: 82\%-84\% using the import list of libraries and used functions, 70\%-80\% using sections, and 83\%-85\% using resources. These findings motivate further investigation into specific variant parts and the development of more sophisticated fingerprinting techniques.



\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/prevalence.pdf}
     \vspace{-0.2cm}
    \caption{File Prevalence.}
    \label{fig:fileprevalnce}
    \vspace{-4mm}
\end{figure}

% \observ{The use of file variation seems very prevalent in the malware field recently. The obtained  results after a thorough analysis of >4 million files, >21 million sections, and >48 million resources suggest that while traditional file hash indicates only 19\% redundancy, digging deeper within file parts, we could see >80\% similarities, which could be significantly useful as first stage triaging mechanism}

\observ{Recent trends in malware show a widespread use of file variation. Analyzing 4 million files, 21 million sections, and 48 million resources, traditional file hashing only identifies $<$ 20\% redundancy. However, deeper analysis of file components reveals over 80\% similarities, highlighting its value as an initial triaging mechanism.}

==> arxive_esorics/sections/5_malware_variation.tex <==
\section{Malware Variation Evasive Methods}\label{sec:malwarevariation}
In this section, we aim to address RQ 2: \textit{What file variation evasive methods can we identify per malware sample?} To achieve this, we first create groups of different malware files exhibiting similar behavior, which we term ``Resilient fingerprints'' (formally defined in Section~\ref{sec:campaginDef}). These groups reveal the evasive methods used. Secondly, we verify the maliciousness of these groups (discussed in Section~\ref{sec:campAnalysis}). Finally, we analyze the identified resilient fingerprints to uncover both variant and invariant parts, detailed in Sections~\ref{sec:variation} and \ref{sec:invariation}.

\subsection{Resilient Fingerprints Definition}\label{sec:campaginDef}
In this section, we introduce the concept of ``\textit{Resilient fingerprints}'', which are sets of PE files sharing the same system functionalities while appearing different at a surface level (i.e., having different file-level hashes). We have found that the most informative aspect of a file that captures its intent is the set of import libraries and the functions they contain, as well as their executable sections, as described in Section~\ref{sec:importList} and illustrated in Figure~\ref{fig:importlist}. These libraries and functions reflect the system functionalities that the file calls upon to perform its actions. For example, the presence of the \textit{Advapi32.dll} library with functions such as \textit{RegCreateKeyExA, RegOpenKeyExA, RegQueryValueExA, and RegSetValueExA} in a file's import libraries would indicate tampering with the Registry. Similarly, the presence of the \textit{KERNEL32.dll} library with functions such as \textit{CopyFileA, CreateFileA, CreateProcessA, CreateThread, and DeleteFileA} would indicate memory and file operations.
Our analysis considers two files to be part of the same resilient fingerprint if they have 100\% similar import libraries and functions, followed by an examination of common executable sections. While these thresholds can be adjusted, this criteria ensures that files must have common executable section code blocks in addition to the import lists to execute that intent, as determined through thorough analysis.

% Note, we have referred to these collections of files with common intent as campaigns, due to the observation that they were submitted to VirusTotal in a similar time frame, and by a diverse group of users, suggesting the existence of coordinated campaigns in the wild. It is also important to note that our focus is not on identifying whether the files in an intent campaign were created by a single attacker, but rather on identifying a set of files with the same intent, which may have been created by one or multiple attackers who leveraged existing sophisticated malware samples.

\vspace{-0.1cm}
\subsection{Resilient Fingerprints Qualitative Analysis}\label{sec:campAnalysis}
 

In this paper, we thoroughly investigate the resilient fingerprints within the four groups' datasets by examining their ground truth labels using data collected from VirusTotal vendors. Our focus in this section is on a qualitative analysis of the top 4-5 resilient fingerprints from each group with a significant number of files (threshold $>=$ 900). To gain a deeper understanding of each resilient fingerprint, we analyze its intent, tag (a simplified version of a unique identifier), type (the operating system file targeted), characteristics (malicious activities), file number (number of files identified with similar import lists and functionalities), longevity (timestamp of the campaign), and file level hash fingerprint (the percentage of identified files with similar file hashes that have been detected using traditional fingerprinting methods such as SHA256).



\subheading{Findings.} We summarize our findings in Table~\ref{tb:topcampaigns}, identifying 18 resilient fingerprints with intents like Worm Autospread, Trojan Zombie, Trojan Spyware, Trojan Mira, and Trojan-Dropper. Noteworthy insights include:
(1) These fingerprints have large sizes, up to 34,068 files, but traditional SHA256 file-level hash fingerprinting methods perform poorly (15 out of 18 cases $<$10\%) in detecting them as similar due to evasion techniques employed by malware authors.
(2) They target both Win32/64 and EXE/DLL, indicating widespread use of evasion tactics.
(3) Some fingerprints date back to 1992 and continue until 2022, highlighting the presence of long-standing malware utilizing known system functionalities that go undetected by traditional fingerprinting mechanisms.
(4) Certain resilient fingerprints reappear in multiple dataset groups, such as Worm Autospread with ID 35b0 (marked in pink) and Trojan Mira with ID 3a58 (marked in green), consistently ranking among the largest identified resilient fingerprints in most of the four groups. Additionally, Trojan Spyware with ID 25ca (marked in orange) and Trojan Spyware with ID 834c (marked in purple), appear across the first/second and second/third groups.


\subheading{Maliciousness Ground Truth.} 
Before delving into the variant evasive and invariant parts of the files in a campaign, it's crucial to establish their maliciousness through other means due to the low effectiveness of traditional hash fingerprinting methods. In this study, we use the vendors' labels within the dataset to determine this ground truth. We calculate the number of vendors labeling each file as malicious, represented as $x$, and create a vector per resilient fingerprint, $r={x_1,x_2,...,x_n}$, where $x_1$ represents file 1, $x_2$ represents file 2, and so on. We then analyze the histogram distribution of $r$. Figure~\ref{fig:groundTruthG} in Appendix \ref{appendix:18fingerprints} displays the maliciousness of ground truth labeling for the top 18 resilient fingerprints. It's evident that all files within each resilient fingerprint are highly malicious, with over 20 vendors labeling them as such.

%Before investigating the variant evasive and invariant parts within the files of an identified campaign, it is necessary to establish the ground truth of maliciousness through other means, as traditional hash fingerprinting methods have a low similarity detection score. In this study, we leverage the vendors' labels within the collected groups' dataset to establish this ground truth.We determine the number of vendors that labeled each file as malicious, $x$, and construct a vector per resilient fingerprint, $r={x_1,x_2,...,x_n}$, where $x_1$ represents file 1, $x_2$ represents file 2, and so on. We then calculate the histogram distribution of $r$. Figure~\ref{fig:groundTruthG} in Appendix \ref{appendix:18fingerprints} shows the maliciousness of ground truth labelling from VirusTotal vendors to the top 18 identified resilient fingerprints. It is clear from the x-axis that all files within each resilient fingerprint are highly malicious, as $>$ 20 vendors have labelled them as malicious.  



% \usepackage{colortbl}


\begin{table}
\centering
\caption{Top  resilient fingerprints from the four groups.}
\label{tb:topcampaigns}
%\vspace{-0.3cm}
\resizebox{4.5in}{!}{
\begin{tabular}{c|c|c|c|c|c|c} 
\hline
\multicolumn{7}{c}{\textbf{Group 1}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ 
\hline
\rowcolor[rgb]{0.937,0.937,0.937} \textbf{Intent}                                                                                            & \textbf{ID}                                                   & \textbf{Type} & \textbf{Characteristics}                                                            & \textbf{Files No}           & \textbf{Longevity}             & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.937,0.937,0.937}}c@{}}\textbf{File Hash }\\\textbf{ Fingerprint}\end{tabular}  \\ 
\hline
{\cellcolor[rgb]{1,0.8,0.788}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{1,0.8,0.788}}c@{}}Worm \\ Autospread\end{tabular}                      & \multicolumn{1}{l|}{{\cellcolor[rgb]{1,0.8,0.788}}35b0}       & Win32.exe     & \begin{tabular}[c]{@{}c@{}}Spread through \\ removables like USB\end{tabular}       & 27,091                      & 1999-2022                      & 3.7\%                                                                                                                    \\ 
\hline
\begin{tabular}[c]{@{}c@{}}Trojan \\ Zombie\end{tabular}                                                                                     & \multicolumn{1}{l|}{8a9e}                                     & Win32.exe     & \begin{tabular}[c]{@{}c@{}}Command \\ Control for attacks\end{tabular}              & 24,119                      & 2011-2022                      & 9.7\%                                                                                                                    \\ 
\hline
{\cellcolor[rgb]{1,0.8,0.404}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{1,0.8,0.404}}c@{}}Trojan \\ Spyware\end{tabular}                       & \multicolumn{1}{l|}{{\cellcolor[rgb]{1,0.8,0.404}}25ca}       & Win64.dll     & \begin{tabular}[c]{@{}c@{}}Stealing Banking \\ Credentials\end{tabular}             & 10,295                      & 2015-2022                      & 0.4\%                                                                                                                    \\ 
\hline
{\cellcolor[rgb]{0.769,0.886,0.769}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.769,0.886,0.769}}c@{}}Trojan \\ Mira\end{tabular}              & \multicolumn{1}{l|}{{\cellcolor[rgb]{0.769,0.886,0.769}}3a58} & Win32.dll     & \begin{tabular}[c]{@{}c@{}}Command Control\\ for attacks\end{tabular}               & 3,596                       & 2014-2022                      & 2.6\%                                                                                                                    \\ 
\hline
\begin{tabular}[c]{@{}c@{}}Trojan \\ Dropper\end{tabular}                                                                                    & \multicolumn{1}{l|}{fbc6}                                     & Win64.dll     & Install other Malware                                                               & 917                         & 2020-2022                      & 4.9\%                                                                                                                    \\ 
\hline
\multicolumn{7}{c}{\textbf{Group 2}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ 
\hline
{\cellcolor[rgb]{1,0.8,0.788}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{1,0.8,0.788}}c@{}}Worm \\ Autospread\end{tabular}                      & \multicolumn{1}{l|}{{\cellcolor[rgb]{1,0.8,0.788}}35b0}       & Win32.exe     & \begin{tabular}[c]{@{}c@{}}Spread through \\ removables like USB\end{tabular}       & \multicolumn{1}{l|}{34,045} & \multicolumn{1}{l|}{1999-2022} & 7.4\%                                                                                                                    \\ 
\hline
Trojan Ransomeware                                                                                                                           & d66e                                                          & Win32.exe     & Encrypt files.                                                                      & 31,747                      & 2008-2022                      & 77.7\%                                                                                                                   \\ 
\hline
{\cellcolor[rgb]{0.796,0.808,0.984}}Trojan Spyware                                                                                           & {\cellcolor[rgb]{0.796,0.808,0.984}}834c                      & Win64.dll     & Keylogger.                                                                          & 17,379                      & 1992-2022                      & 3.0\%                                                                                                                    \\ 
\hline
{\cellcolor[rgb]{0.769,0.886,0.769}}Trojan Mira                                                                                              & {\cellcolor[rgb]{0.769,0.886,0.769}}3a58                      & Win32.dll     & \begin{tabular}[c]{@{}c@{}}Remote Command \\ Control\end{tabular}                   & 10,794                      & 2014-2022                      & 3.1\%                                                                                                                    \\ 
\hline
{\cellcolor[rgb]{1,0.8,0.404}}Trojan Spyware                                                                                                 & {\cellcolor[rgb]{1,0.8,0.404}}25ca                            & Win64.dll     & \begin{tabular}[c]{@{}c@{}}Stealing banking \\ credentials.\end{tabular}            & 2,070                       & 2015-2022                      & 5.2\%                                                                                                                    \\ 
\hline
\multicolumn{7}{c}{\textbf{Group 3}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ 
\hline
{\cellcolor[rgb]{1,0.8,0.788}}Worm Autospread                                                                                                & {\cellcolor[rgb]{1,0.8,0.788}}35b0                            & Win32.exe     & \begin{tabular}[c]{@{}c@{}}Spread through \\ removables like USB\end{tabular}       & 34,068                      & 1992-2022                      & 5.6\%                                                                                                                    \\ 
\hline
Virus Fujaks                                                                                                                                 & 9dab                                                          & Win32.exe     & \begin{tabular}[c]{@{}c@{}}Prevent security \\ processes from running.\end{tabular} & 20,844                      & 1992-2022                      & 3.0\%                                                                                                                    \\ 
\hline
{\cellcolor[rgb]{0.796,0.808,0.984}}Trojan Spyware                                                                                           & {\cellcolor[rgb]{0.796,0.808,0.984}}834c                      & Win64.dll     & Keylogger.                                                                          & 18,068                      & 1992-2022                      & 2.8\%                                                                                                                    \\ 
\hline
{\cellcolor[rgb]{0.769,0.886,0.769}}Trojan Mira                                                                                              & {\cellcolor[rgb]{0.769,0.886,0.769}}3a58                      & Win32.dll     & \begin{tabular}[c]{@{}c@{}}Remote Command \\ Control\end{tabular}                   & 10,232                      & 2014-2022                      & 1.8\%                                                                                                                    \\ 
\hline
\multicolumn{7}{c}{\textbf{\textbf{Group 4 (Collected 9 months after)}}}                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ 
\hline
\multicolumn{1}{c|}{Trojan Ransomeware}                                                                                                     & 5a7b                                                          & Win32.exe     & Encrypt Files                                                                       & 11,926                      & 2008-2022                      & \multicolumn{1}{c}{18.1\%}                                                                                              \\ 
\hline
\multicolumn{1}{c|}{Trojan Malware}                                                                                                         & 6448                                                          & Win32.exe     & \begin{tabular}[c]{@{}c@{}}Remote Command \\Control\end{tabular}                    & 8,842                       & 1992-2022                      & \multicolumn{1}{c}{37.3\%}                                                                                              \\ 
\hline
\multicolumn{1}{c|}{{\cellcolor[rgb]{1,0.8,0.788}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{1,0.8,0.788}}c@{}}Worm \\Autospread\end{tabular}} & {\cellcolor[rgb]{1,0.8,0.788}}35b0                            & Win32.exe     & \begin{tabular}[c]{@{}c@{}}Spread through \\~removables likeUSB~ ~ ~~\end{tabular}  & 1,979                       & 1992-2022                      & \multicolumn{1}{c}{6.7\%}                                                                                               \\ 
\hline
\multicolumn{1}{c|}{{\cellcolor[rgb]{0.769,0.886,0.769}}Trojan Mira}                                                                        & {\cellcolor[rgb]{0.769,0.886,0.769}}3a58                      & Win32.dll     & \begin{tabular}[c]{@{}c@{}}Remote Command\\Control\end{tabular}                     & 1,969                       & 2003-2022                      & \multicolumn{1}{c}{10.6\%}                                                                                              \\
\hline
\end{tabular}}
\end{table}


\subsection{Reliable Invariant  Executable Parts}\label{sec:invariation}
%\sharif{Add one importlist as graph representation as an example!}

\subheading{Findings.} 
After analyzing the files' critical components, we find that the identified resilient fingerprints share common executable section blocks. We categorize these into three types: ``Malicious'', ``Standard'', and ``Camouflage''. The ``Malicious'' section contains most of the malicious code, characterized by high entropy ($>$5) and frequent obfuscation. The ``Standard'' section contains generic standard operation code blocks with normal entropy ($\leq5$), possibly called by the ``Malicious'' section. The ``Camouflage'' section, with an entropy of 0 and a small raw size ($<$4096 bytes), appears to be a padding section with automatically generated continuous characters. These characteristics are consistent across all four groups.\\

%After thoroughly analysing the files' critical components, we discover that the identified resilient fingerprints utilize common executable section blocks. Specifically, we identify three types of invariant sections, and named them ``Malicious'', ``Standard'', and ``Camouflage''. The ``Malicious'' section is where the majority of malicious code is embedded, characterized by high entropy ($>$5) and frequent obfuscation. The ``Standard'' section appears to contain generic standard operation code blocks that may be called by the ``Malicious'' section and has normal entropy ($\leq5$). The ``Camouflage'' section is the most intriguing aspect we identified. It appears to be a padding section with an entropy of 0 and a small raw size ($<$4096 bytes), indicating the presence of automatically generated continuous characters. These findings were prevalent across all four groups.\\ 

\subheading{Results Insight 1.} Table~\ref{tb:invariationSec} details the invariant sections for the resilient fingerprint ``Worm Autospread'' (ID 35b0), observed in all four groups. Each section is identified by a SecID, a shortened version of its content hash. The table includes entropy, count, and our analysis label for each section in the fingerprint files across the groups. These sections are consistently present not only within each group but also across multiple groups. Among the five identified sections, two are likely ``Malicious'', two are ``Standard'', and one is ``Camouflage''.

%Table~\ref{tb:invariationSec} provides a detailed examination of the invariant sections for the resilient fingerprint ``Worm Autospread'' (ID 35b0), which was observed across all four groups. This resilient fingerprint consists of five sections, each identified by a SecID, which is a shortened version of the first and last two characters of their content hash. The table also includes the entropy and count of each section within the fingerprint files for each group, as well as our analysis label. It is evident that these sections are present not only within the resilient fingerprint for each group dataset, but also across multiple groups. Out of the five sections, we can see that this resilient fingerprint includes two likely ``Malicious'', two ``Standard'', and one ``Camouflage'' sections.

\begin{table}[h]
\caption{Invariant Sections. Zoom in to Worm Autospread resilient fingerprint with ID 35b0.}
%\vskip2pt
\label{tb:invariationSec}
%\vspace{-0.3cm}
\centering
\resizebox{2.8in}{!}{
\begin{tabular}{c|c|c|c|c|c|c}
\hline
{\bf SecID} & {\bf Entropy} & \begin{tabular}[c]{@{}c@{}}{\bf Count}\\ {\bf Group 1}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\bf Count}\\ {\bf Group 2}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\bf Count}\\ {\bf Group 3}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\bf Count}\\ {\bf Group 4}\end{tabular} & {\bf Label}      \\ \hline
d47e  & 0       & 27103                                                   & 34045                                                   & 34262                                                &2179   & Camouflage \\ \hline
31d3  & 7.89    & 15411                                                   & 16158                                                   & 17313                                                 &--   & Malicious  \\ \hline
80b1  & 2.81    & 15411                                                   & 16158                                                   & 17313                                                 &986   & Standard   \\ \hline
40af  & 7.91    & 11692                                                   & 17887                                                   & 16949                                                 &1193   & Malicious  \\ \hline
3a56  & 2.79    & 11692                                                   & 17887                                                   & 16949                                                 &1193   & Standard   \\ \hline
\end{tabular}}
\end{table}

\subheading{Results Insight 2.} Table~\ref{tb:invariationSec2} presents the invariant sections of the ``Trojan Spyware'' resilient fingerprint (ID 25ca), observed in groups 1 and 2 of our datasets. This fingerprint, in addition to the patterns discussed in Insight 1, reveals extensive use of camouflage sections by the malware authors. Out of the ten sections, four are camouflage, characterized by an entropy of 0 and simple padding of $<$4096 bytes. Moreover, the malwre authors repeatedly include the same camouflage section within a single malware sample. For instance, SecID ``d47e'' appeared 157,453 times across 10,295 files, averaging around 12-15 copies per file. These tactics, besides altering file hashes, likely serve to increase the size of malicious files, adding complexity to subsequent static and dynamic analyses.

%Table~\ref{tb:invariationSec2} examines the invariant sections of another resilient fingerprint, ``Trojan Spyware'' (ID 25ca), which was observed twice across groups 1 and 2 of our datasets. In addition to the patterns discussed in Insight 1 regarding the three common sections, this fingerprint reveals that the malware authors also extensively utilize camouflage sections. For instance, four of the ten sections are camouflage, characterized by an entropy of 0 and simple padding of <4096 bytes. Additionally, the malware authors repeatedly include the same camouflage section within the same malware sample. For instance, SecID ``d47e'' appeared 157,453 times across 10,295 files or around 12-15 copies per file. These tactics, beyond altering the file hashes, are likely used also to increase the size of the malicious files, making it more challenging for the next stage of static and dynamic analysis.

\begin{table}[h]
\caption{Invariant Sections. Focus on Trojan Spyware resilient fingerprint with ID 25ca/10295 files.}
%\vskip2pt
\label{tb:invariationSec2}
%\vspace{-0.3cm}
\centering
\resizebox{2.1in}{!}{
\begin{tabular}{c|c|c|c|c}
\hline
{\bf SecID} & {\bf Entropy} & \begin{tabular}[c]{@{}c@{}}{\bf Count}\\ {\bf Group 1}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\bf Count}\\ {\bf Group 2}\end{tabular} & {\bf Label}      \\ \hline
6210  & 0       & 157453                                                  & 33183                                                   & Camouflage \\ \hline
0822  & 0       & 83165                                                   & 17294                                                   & Camouflage \\ \hline
459b  & 0       & 12326                                                   & 2584                                                    & Camouflage \\ \hline
b66c  & 5.14    & 10295                                                   & 2070                                                    & Malicious  \\ \hline
a214  & 2.78    & 10295                                                   & 2070                                                    & Standard   \\ \hline
ca9d  & 4.04    & 10295                                                   & 2070                                                    & Standard   \\ \hline
bad4  & 0       & 10295                                                   & 2070                                                    & Camouflage \\ \hline
0e5c  & 4.09    & 10295                                                   & 2070                                                    & Standard   \\ \hline
07aa  & 7.82    & 10290                                                   & 2069                                                    & Malicious  \\ \hline
21ae  & 6.67    & 10290                                                   & 2069                                                    & Malicious  \\ \hline
\end{tabular}}
\end{table}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/variant_campaign1_1.pdf}
     %\vspace{-0.3cm}
    \caption{Section Numbers, Virtual Size, and Address variant.}
    \label{fig:variantSize_sections}
    \vspace{-4mm}
\end{figure}


\subsection{Unreliable Invariant non-Executable Parts}\label{sec:resourcesUnrialiable}

\subheading{Findings.} After a thorough investigation, we have discovered that many resilient fingerprints clusters are formed based on imported libraries and show high similarity in non-executable resources like images and logos. However, unlike section code blocks, the presence of resource-based clusters does not always imply malicious intent. This is because these resources, such as Microsoft logos, can be used by both benign and malware samples (see Appendix \ref{appendix:unreliableParts} for details).\\

%Following a comprehensive investigation, we have found that several of the identified resilient fingerprints clusters are based on the imported libraries and have high similarity in the non-executable resources, such as images and logos. However, unlike the section code blocks, the presence of resource-based clusters does not necessarily indicate malicious intent. This is because these resources, such as Microsoft logos, may be used by both benign and malware samples (See Appendix \ref{appendix:unreliableParts} for results).\\



\subsection{Variant Evasive Parts}\label{sec:variation}
\subheading{Findings.} Our analysis of resilient fingerprint files reveals various tactics employed by malware authors to evade detection and hide their file hash fingerprints. These tactics focus on section numbers, virtual size, virtual address, and section names. (1) Malware authors frequently use high section numbers to inject camouflage sections and increase file size, making analysis more challenging. (2) Manipulating virtual size by utilizing uninitialized arrays in specific sections alters the memory size footprint. (3) The virtual address, the location in memory where the file is loaded, is also manipulated by loading the same sections into random memory locations. (4) Additionally, malware authors use variant section names to conceal common sections with identical content. The subsequent presentation provides evidence and results supporting these findings.\\

% Our analysis of multiple resilient fingerprint files revealed that malware authors employ various tactics to evade detection and conceal their file hash fingerprints. Specifically, we identify four key areas in which these tactics are employed: section numbers, virtual size, virtual address, and section names.
% Regarding section numbers, we find that malware authors often use high numbers to inject camouflage sections and increase the file size, making it more difficult to process during static or dynamic analysis. Virtual size, which refers to the size of the file when loaded into memory, can also be manipulated by using uninitialized arrays in certain sections, resulting in different memory size footprints.
% Virtual address, which refers to the location in memory where the file is loaded, can also be manipulated by malware authors, who may load the same sections into various random locations in memory. Finally, we find that malware authors often use variant section names to camouflage common sections with identical content, another tactic used to evade detection.
% In the following, we present evidence and results that support these findings.\\


\subheading{Results Insight 1.} As shown in Figure~\ref{fig:variantSize_sections}. (c), the distribution of section numbers within the Trojan Spyware (ID 25ca) resilient fingerprint, which comprises 10,295 files and over 300,000 sections, reveals significant variability. Despite the presence of invariant section blocks, as previously discussed, the number of sections per file varies considerably, ranging from 10 to 50. A large proportion of these sections are attributed to camouflage sections (SecID 6210 and 0822, as shown in Table~\ref{tb:invariationSec2}), which are mostly empty sections.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.60\linewidth]{figures/sectionNo_C1_10295.pdf}
%      % \vspace{0.2cm}
%     \caption{The distribution of section numbers within 10,295 files of resilient fingerprint Trojan Spyware.}
%     \label{fig:sectionNo}
%     %\vspace{-8mm}
% \end{figure}

\subheading{Results Insight 2.}  As Figure~\ref{fig:variantSize_sections}. (a) and (b)  illustrates that virtual size is highly variable among resilient fingerprint files, despite the presence of identical section content. This variability ranges from 0 to 3,500. Similarly, the virtual address is widely dispersed, ranging from 0.1e6 to 1.6e6. Additionally, Figure~\ref{fig:secion_names} in Appendix \ref{appendix:sectionNames} exhibits that the section names (with identical content) display high randomness, suggesting that they were auto-generated as a camouflage tactic.\\

It is important to note that the degree of variability across the variant parts we have discussed varies among fingerprints. Some resilient fingerprints may exhibit a higher degree of randomness in certain areas, such as section numbers, virtual addresses, virtual sizes, or section names, while others may exhibit less variability in these areas. To aid the reviewers further, we have made all identified top resilient fingerprints available in our repository at ~\url{https://github.com/anonymousConfer/malware\_fingerprint}.








\observ{Import libraries with lists of functionalities and executable section blocks are reliable components for identifying invariant parts of malware samples through resilient fingerprints. Evasive methods used by malware include altering the number of sections, virtual size, virtual address, section names, and occasionally code size variations.}

==> arxive_esorics/sections/6_improve_fingerprint.tex <==
\section{Fingerprint detection Improvement}\label{sec:detectionimprovment}
This section addresses RQ3: \textit{How can malware fingerprinting be improved?} We propose two approaches, ``Top-Down'' and ``Bottom-Up'', leveraging the hierarchical structure of file metadata, which ranges from import libraries at the highest level to executable section blocks at the lowest. By exploiting this structure, we aim to identify resilient and invariant similarities, starting from the top and moving downwards. In the following subsections, we detail both approaches, including the algorithms used, and present our investigation results.

%This section focuses on answering RQ3: \textit{How to improve malware fingerprinting?} To achieve this, we put forth two approaches named ``Top-Down'' and ``Bottom-Up''. The underlying idea revolves around the structured nature of file metadata, which forms a tree-like hierarchy from the highest level (import libraries) to the lowest level (executable section blocks), encompassing lists of functionalities. Exploiting this structure, we aim to identify the resilient and invariant path of similarities, starting from the top and progressing towards the bottom. In the subsequent subsections, we delve into both approaches, providing comprehensive descriptions of the algorithms employed. Furthermore, we present the results obtained from our investigations.

%We propose two approaches called ``Top-Down'' and ``Bottom-up''. The intuition here is that as the file metadata is structured as a tree from top to bottom presenting import libraries with a List of functionalities, and executable sections, we use that to identify the resilient path of similarities from the top (import libraries) to the bottom (actual executable section blocks).   In the following subsections, we discuss both approaches and present both algorithms and their descriptions. We follow by presenting the obtained results. 

% \todo[inline,size=\small, color=blue!40]{Focus on 2 approaches. Top to bottom. Bottom-to-top approaches. Their relevant algorithms and results}

% Started various clustering strategies 
% Developing reliable mechanism

% \subsection{Preprocessing}
% To streamline our algorithmic process, we reorganise the data collected from VirusTotal feeds into entity-relation structures. The first table contains high-level metadata about each file, while the second table contains detailed information about each file's sections, including content hash, entropy, and other relevant details. The relationship between these two tables is one-to-many, meaning that each feed can have multiple entries in the section's data structure, reflecting the various sections that comprise the file.

\subsection{Top-Down Approach}

The Top-Down approach initially clusters resilient fingerprints based on 100\% similarities in their import libraries and functionalities. Subsequently, it conducts a detailed analysis of the sections within these resilient fingerprints, focusing on identifying malicious or camouflage sections. This analysis creates comprehensive profiles for each resilient fingerprint, encompassing detailed statistics at both the file and section levels to assess the likelihood of a file belonging to a resilient fingerprint.

%To detect and evaluate potential resilient fingerprints, the Top-down approach first clusters resilient fingerprints based on 100\% similarities in their import libraries and functionalities. Next, we conduct a detailed analysis of the sections in these resilient fingerprints, with a particular focus on identifying any malicious or camouflage sections. Based on this analysis, we create a comprehensive profile for each resilient fingerprint, including detailed statistics at both the file and section levels. By analyzing these statistics, we can determine the likelihood that a given file belongs to a resilient fingerprint.

Algorithm~\ref{algo1:top-down} outlines the top-down process. It takes two separate parameters, $\texttt\it{{feeds}}$ and $\texttt\it{{sections}}$, and groups the feeds by their import list similarity $\texttt\it{{imphash}}$. The groups are then sorted in descending order based on their count, allowing us to focus on the significant clusters first (steps 1-2). Next, we iterate through each cluster in $\texttt\it{{SortimpLists}}$, using each entry's $\texttt\it{{imphash}}$ to locate all relevant files from $\texttt\it{{feeds}}$. We then calculate file-level statistics, such as entropy and hashes (steps 4-6). We also dive into $\texttt\it{{sections}}$ to retrieve all the sections that belong to the resilient fingerprint, group those sections using $\texttt\it{{secHash}}$, and sort them in descending order based on count to prioritize significant sections (steps 7-9). We then iterate through each cluster of sections within $\texttt\it{{sortsecKeys}}$, using each entry's $\texttt\it{{secKey}}$ to locate all relevant sections before collecting all the statistics about that common section (steps 12-13). For example, if we have ten sections with similar keys, we collect the minimum and maximum entropy, and minimum and maximum chi-squared distance (Chi2). We decide to focus on the top 10 sections within each resilient fingerprint as a threshold. Finally, we combine the collected $\texttt\it{{feedsInfo}}$ and $\texttt\it{{section[]}}$ to create $\texttt\it{{resilientFprintInfo}}$, which forms the basis of our decision-making process.



\begin{algorithm}[!ht]
%\algsetup{linenosize=\tiny}
\scriptsize
\caption{Top-Down Approach}\label{algo1:top-down}
\begin{algorithmic}[1]
\Statex \textbf{Input: } $\texttt{feeds},\texttt{sections}$ \Comment{$feeds: f_1,f_2..,f_n. sections: s_1,s_2..,s_n$} %\text{f_1,f_2,..,f_n}, \texttt{sections} \text{s_1,s_2,..,s_n}$
\Statex \textbf{Output: } $\texttt{resilientFprintInfo}$ \Comment{set of resilient fingerprints, each has related meta-info}
\State $\texttt{impLists}$ = group \texttt{feeds} by \texttt{imphash}  \Comment{imphash is unique identifier for import list}
\State $\texttt{SortimpLists}$ = sort $\texttt{impLists}$ by count in descending order  
\State $\texttt{resilientFprintInfo}$ = []  
\For{$\texttt{imphash}$ in $\texttt{SortimpLists}$}
\State $\texttt{resilientFingerprints{[]}}$ = locate $\texttt{feeds}$  by $\texttt{imphash}$
\State $\texttt{feedsInfo}$ = calculate $\texttt{resilientFingerprints{[]}}$  stats
\State $\texttt{RFprintSections}$ = locate relevant $\texttt{sections}$  of $\texttt{resilientFingerprints{[]}}$
\State $\texttt{secKeys}$ = group $\texttt{RFprintSections}$ by $\texttt{secHash}$  \Comment{secHash is unique section identifier}
\State $\texttt{sortsecKeys}$ = sort $\texttt{secKeys}$ descendingly by count  
\State $\texttt{secInfo}$ = [] 
\For{$\texttt{secKey}$ in $\texttt{sortsecKeys}$}
\State $\texttt{section{[]}}$ = locate $\texttt{RFprintSections}$  by $\texttt{secKey}$
\State $\texttt{sparams}$ = calculate $\texttt{section{[]}}$  stats
\State append $\texttt{sparams}$ to $\texttt{secInfo}$
\EndFor
\State append $\texttt{feedsInfo}$,$\texttt{section{[]}}$,$\texttt{secInfo{[]}}$ to  $\texttt{resilientFprintInfo}$
\EndFor
\end{algorithmic}
\end{algorithm}




% \usepackage{multirow}
% \usepackage{colortbl}


% \usepackage{multirow}
% \usepackage{colortbl}




% \usepackage{multirow}
% \usepackage{colortbl}


% \usepackage{multirow}
% \usepackage{colortbl}



% \usepackage{multirow}
% \usepackage{colortbl}




\subsection{Bottom-Up Approach}
This approach is going the other way around to start from the bottom up by clustering all files that use common sections, including camouflage or malicious. This approach is motivated by our analysis, where we find that common camouflage sections and malicious sections could be found in another resilient fingerprint that has different import list libraries when we follow the Top-Bottom approach. We attribute that to  Malware authors slightly manipulating the import list libraries to avoid being detected or using the same executable sections for different intent. Therefore, starting from the bottom (sections) up, we can capture resilient fingerprints robust to slight import variations. Similar to the previous approach, a profile is built to determine the maliciousness of the fingerprints.

Algorithm~\ref{algo2:bottom-up} outlines the bottom-up process. It takes two similar separate parameters, $\texttt\it{{feeds}}$ and $\texttt\it{{sections}}$ of the entire group (1M feeds and their sections). We begin by diving into $\texttt\it{{sections}}$ to retrieve all common sections, group those sections using $\texttt\it{{secHash}}$, and sort them in descending order based on count to prioritize significant sections (steps 1-2). We then iterate through each cluster of sections within $\texttt\it{{sortsecKeys}}$, using each entry's $\texttt\it{{secKey}}$ to locate all relevant sections (steps 4-5). Next, we use collected $\texttt\it{{RFprintSections[]}}$ to go up to the file level and retrieve all relevant file-level feeds (steps 6). We observe here that we might encounter redundant file-level feeds as multiple sections might belong to the same file and cause double dipping counting. Hence, we introduce step 7 as a filtering condition to eliminate this redundancy using $\texttt\it{{feedID}}$ before collecting all the statistics about that common section (steps 8-9).



\begin{algorithm}[!h]
%\algsetup{linenosize=\tiny}
\scriptsize
\caption{Bottom-Up Approach}\label{algo2:bottom-up}
\begin{algorithmic}[1]
\Statex \textbf{Input:} $\texttt{feeds},\texttt{sections}$ \Comment{$feeds: f_1,f_2..,f_n. sections: s_1,s_2..,s_n$}
\Statex \textbf{Output:} $\texttt{resilientFprintInfo}$\Comment{set of resilient fingerprints, each  has related meta-info}
\State $\texttt{secKeys}$ = group $\texttt{sections}$ by $\texttt{secHash}$  \Comment{secHash is unique identifier}
\State $\texttt{sortsecKeys}$ = sort $\texttt{secKeys}$ descendingly by count
\State $\texttt{resilientFprintInfo}$ = []  
\For{$\texttt{secKey}$ in $\texttt{sortsecKeys}$}
\State $\texttt{RFprintSections{[]}}$ = locate $\texttt{sections}$  by $\texttt{secKey}$
\State $\texttt{resilientFprint{[]}}$ = locate $\texttt{feeds}$  by $RFprintSections{[]}$
\State $\texttt{resilientFprint{[]}}$ = drop duplicates $resilientFprint{[]}$  by $\texttt{feedsID}$
\State $\texttt{sparams}$ = calculate $\texttt{RFprintSections{[]}}  \text{stats}$
\State $\texttt{fparams}$ = calculate $\texttt{resilientFprint{[]}} \text{stats}$
\State append $\texttt{sparams}$,$\texttt{fparams}$ to  $\texttt{resilientFprintInfo}$
\EndFor
\end{algorithmic}
\end{algorithm}



% \usepackage{multirow}
% \usepackage{colortbl}


% \usepackage{multirow}
% \usepackage{colortbl}




\subsection{Results}
\subheading{Overview and settings.} 
We derive statistical heuristics for both approaches as detailed in Algorithms \ref{algo1:top-down} and \ref{algo2:bottom-up}. In the results section, we explore various combinations across our four datasets' groups to assess their potential efficacy, including Import List (IL), Redundant Sections (RS), Camouflage Sections (CS), and Malicious Sections (MS) as defined in Invariant Parts (Section\ref{sec:invariation}). We use vendors' labels as ground truth for evaluating the maliciousness of identified fingerprints. We employ a conservative threshold ($t \geq 4$) to indicate a binary as malicious. We also refer to the number of files within a resilient fingerprint as redundancy. The accuracy column reflects our approach's effectiveness in identifying files and determining their likelihood of association with a resilient fingerprint, rather than binary classification between benign and malware.

We categorize resilient fingerprints into three types: \textit{\underline{fully malicious}}, where all files are flagged by four or more vendors as malicious; \textit{\underline{false positives (FP)}}, where all files are flagged by fewer than four vendors; and \textit{\underline{partial malicious}} (most intersting), where some files are highly flagged by vendors while others are not, yet they share common import lists and camouflage or malicious section blocks. We combine these categories to assess true positive (TP) accuracy. The following results provide more details with a specific focus on FP and TP. Note that all thresholding is derived from group 1, and we use groups 2, 3, and 4 to assess the generalizability of our findings.\\


\subheading{Top-Down Results.}
We analyze the Top-Down approach using five combinations across four groups. The results in Table~\ref{tb:top-downDetection} are as follows. (1) IL and RS combination: Identify approximately 560 fingerprints with a high FP rate (around 6.8\%) and a TP rate of about 93.1\%. Consistent results are observed across all four groups, with slightly higher FP (9\%) and lower TP (90\%). 
(2) IL and CS combination: Reduce the number of identified fingerprints by more than half, resulting in improved FP rates (between 1.3\% and 2.8\%) and TP rates (between 97.1\% and 98.6\%). Identify around 25\% of 1 million files within each group.
(3) IL and MS combination: Increase the total number of identified resilient fingerprints to two-thirds. Reasonable FP rates (between 2.2\% and 3.9\%) and TP rates (between 96\% and 97.7\%) are achieved, identifying around 323K-434K of all 1 million files within each group.
(4) IL, CS, and MS combination: Among all combinations, it has one of the lowest numbers of identified resilient fingerprints (between 195-347). However, it provides decent FP rates (between 1.3\% and 2.8\%) and TP rates (between 97.1\% and 98.6\%), identifying between 213K-227K of all files within each group. This combination is considered too strict.
(5) Based on these observations, the fifth combination of IL and either CS or MS proves to be the most effective. It identifies the highest number of resilient fingerprints (between 345 and 1025) with FP rates (between 2.2\% and 3.9\%) and TP rates (between 96\% and 97.7\%). It identifies slightly more files (between 324K-339K), representing approximately 33\% of all 1 million files within each group. Thus, the presence of IL, combined with either CS or MS, is deemed sufficient to connect a file to a resilient fingerprint. 
%Figure~\ref{fig:top_campaigns} illustrates the sizes of the top 20 identified resilient fingerprints, ranging from 10,000 to 60,000 per fingerprint.
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/top_fingerprints.pdf}
%      % \vspace{0.2cm}
%     \caption{The number of files in the top 20 detected Top-Down  resilient fingerprints.} 
%     \label{fig:top_campaigns}
%     %\vspace{-8mm}
% \end{figure}

% We analyze the Top-Down approach using five combinations across four groups, and the detailed results are presented in Table~\ref{tb:top-downDetection}. First, we examine the combination of IL and RS, which had the highest number of identified campaigns (approximately 560) but resulted in a high FP rate (around 6.8\%) and a TP rate of about 93.1\%, identifying 544,614 out of 1,061,151 (50\%) of the files. The results were consistent across all three groups, with slightly higher FP (9\%) and lower TP (90\%). Second, we combine IL with CS, which reduce the number of identified campaigns by more than half but resulted in a significant improvement in both the FP rate (between 1.3\% and 2.8\% across the groups) and the TP rate (between 97.1\% and 98.6\% across the groups), identifying around 25\% of all files within each group. 
% %
% Third, we evaluate the combination of IL and MS, which increase the total number of identified resilient fingerprints to two-thirds with a reasonable FP rate (between 2.2\% and 3.9\% across the groups) and TP rate (between 96\% and 97.7\% across the groups), identifying around 323K-434K of all 1 million files within each group. Fourth, we combine IL, CS, and MS, which has one of the lowest total numbers of identified resilient fingerprints (between 195-347 across the groups) among all combinations. However, it still provides a decent FP rate (between 1.3\% and 2.8\% across the groups) and TP rate (between 97.1\% and 98.6\% across the groups), identifying between 213K-227K of all files within the 1 million in each group. We observe that this combination was too strict, and it was unlikely that malware writers would use the camouflage and malicious sections simultaneously most of the time.

% Based on this observation, we examine the fifth combination of IL and either CS or MS, which seem to be the most effective in terms of the total number of identified resilient fingerprints (between 345 and 1025 across the groups), the FP rate (between 2.2\% and 3.9\% across the groups), and the TP rate (between 96\% and 97.7\% across the groups), identifying slightly more files between 324K-339K (approximately 33\%) of all 1 million files within each group. Therefore, it is reasonable to conclude that the presence of IL, in addition to either CS or MS, is sufficient to connect a file to a resilient fingerprint.

\begin{table}[h]
\centering
\caption{Top-Down Approach resilient Fingerprinting.}
\label{tb:top-downDetection}
%\vspace{-0.3cm}
\resizebox{4.4in}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{Top-Down}                & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ Fingerprint\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\\ (F\textless{}4 )\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\\ ( F\textless{}4,F\textgreater{}=4 )\end{tabular} & \begin{tabular}[c]{@{}c@{}}\\ (F\textgreater{}=4)\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}\\ (TP)\end{tabular}}  \\ 
\cline{3-9}
                                         &                                                                         & Num & Acc.(\%) & Redundancy                                                           & \multicolumn{2}{c|}{Num}                                                                                                                        & Acc.(\%) & Redundancy                                                      \\ 
\hline
\multicolumn{9}{|c|}{Group 1}                                                                                                                                                                                                                                                                                                                                                                                                   \\ 
\hline
ILRS                                     & 560                                                                     & 51  & 6.8      & 40,034                                                          & 158                                                                            & 351                                                            & 93.1     & 544,613                                                    \\ 
\hline
ILCS                                     & 222                                                                     & 11  & 1.3      & 3,070                                                           & 67                                                                             & 144                                                            & 98.6     & 224,803                                                    \\ 
\hline
ILMS                                     & 394                                                                     & 32  & 2.2      & 7,572                                                           & 103                                                                            & 261                                                            & 97.7     & 335,062                                                    \\ 
\hline
ILCSMS                                   & 219                                                                     & 11  & 1.3      & 3,070                                                           & 66                                                                             & 142                                                            & 98.6     & 223,513                                                    \\ 
\hline
\rowcolor[rgb]{0.867,1,0.867} ILCS(or)MS & 345                                                                     & 22  & 2.2     & 7,572                                                           & 95                                                                             & 231                                                            & 97.7     & 339,278                                                    \\ 
\hline
\multicolumn{9}{|c|}{Group 2}                                                                                                                                                                                                                                                                                                                                                                                                   \\ 
\hline
ILRS                                     & 478                                                                     & 56  & 9.0      & 53,682                                                          & 148                                                                            & 274                                                            & 90.9     & 540,439                                                    \\ 
\hline
ILCS                                     & 197                                                                     & 13  & 2.0      & 4,407                                                           & 67                                                                             & 117                                                            & 97.9     & 213,656                                                    \\ 
\hline
ILMS                                     & 344                                                                     & 39  & 2.9      & 9,993                                                           & 97                                                                             & 208                                                            & 97.0     & 323,728                                                    \\ 
\hline
ILCSMS                                   & 195                                                                     & 13  & 2.0      & 4,407                                                           & 66                                                                             & 116                                                            & 97.9     & 213,021                                                    \\ 
\hline
\rowcolor[rgb]{0.867,1,0.867} ILCS(or)MS & 346                                                                     & 39  & 2.9      & 9,993                                                           & 98                                                                             & 209                                                            & 97.0     & 324,363                                                    \\ 
\hline
\multicolumn{9}{|c|}{Group 3}                                                                                                                                                                                                                                                                                                                                                                                                   \\ 
\hline
ILRS                                     & 494                                                                     & 62  & 9.3      & 56,581                                                          & 144                                                                            & 288                                                            & 90.6     & 548,525                                                    \\ 
\hline
ILCS                                     & 196                                                                     & 17  & 2.8      & 6,499                                                           & 61                                                                             & 118                                                            & 97.1     & 218,264                                                    \\ 
\hline
ILMS                                     & 355                                                                     & 43  & 3.4      & 11,753                                                          & 93                                                                             & 219                                                            & 96.5     & 329,789                                                    \\ 
\hline
ILCSMS                                   & 195                                                                     & 17  & 2.8      & 6,499                                                           & 61                                                                             & 117                                                            & 97.1     & 217,782                                                    \\ 
\hline
\rowcolor[rgb]{0.867,1,0.867} ILCS(or)MS & 356                                                                     & 43  & 3.4      & 11,753                                                          & 93                                                                             & 220                                                            & 96.6   & 330,271                                                    \\ 
\hline
\multicolumn{9}{|c|}{Group 4 (Collected 9 months after)}                                                                                                                                                                                                                                                                                                                                                                        \\ 
\hline
ILRS                                     & 1419                                                                    & 88  & 4.3      & 29,309                                                          & 164                                                                            & 1167                                                           & 95.6     & 652,168                                                    \\ 
\hline
ILCS                                     & 351                                                                     & 15  & 2.7      & 6,403                                                           & 15                                                                             & 258                                                            & 97.2     & 229,597                                                    \\ 
\hline
ILMS                                     & 1021                                                                    & 60  & 3.9      & 17,678                                                          & 127                                                                            & 834                                                            & 96.0     & 434,068                                                    \\ 
\hline
ILCSMS                                   & 347                                                                     & 14  & 2.6      & 6,236                                                           & 78                                                                             & 255                                                            & 97.3     & 227,134                                                    \\ 
\hline
\rowcolor[rgb]{0.867,1,0.867} ILCS(or)MS & 1025                                                                    & 61  & 3.9      & 17,845                                                          & 127                                                                            & 837                                                            & 96.0     & 436,531                                                    \\
\hline
\end{tabular}}
\end{table}


\begin{table}
\centering
\caption{Bottom-Up Approach resilient Fingerprinting.}
\label{tb:bottom-upDetection}
%\vspace{-0.3cm}
\resizebox{4.4in}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{Bottom-Up}             & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ Fingerprint\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\\ (F\textless{}4 )\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\\ ( F\textless{}4,F\textgreater{}=4 )\end{tabular} & \begin{tabular}[c]{@{}c@{}}\\ (F\textgreater{}=4)\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}\\ (TP)\end{tabular}}  \\ 
\cline{3-9}
                                       &                                                                         & Num  & Acc.  (\%) & Redundancy                                                        & \multicolumn{2}{c|}{Num}                                                                                                                        & Acc. (\%) & Redundancy                                                     \\ 
\hline
\multicolumn{9}{|c|}{Group 1}                                                                                                                                                                                                                                                                                                                                                                                                 \\ 
\hline
RS                                     & 603                                                                     & 141  & 5.1        & 34,640                                                       & 187                                                                            & 278                                                            & 94.9      & 656,219                                                   \\ 
\hline
CS                                     & 26                                                                      & 4    & 0.1        & 7                                                            & 21                                                                             & 1                                                              & 99.9      & 457,365                                                   \\ 
\hline
MC                                     & 273                                                                     & 39   & 4.1        & 4,038                                                        & 67                                                                             & 167                                                            & 95.9      & 105,719                                                   \\ 
\hline
\rowcolor[rgb]{0.867,1,0.867} CS(or)MC & 299                                                                     & 43   & 0.8        & 4,448                                                        & 88                                                                             & 168                                                            & 99.2      & 563,084                                                   \\ 
\hline
\multicolumn{9}{|c|}{Group 2}                                                                                                                                                                                                                                                                                                                                                                                                 \\ 
\hline
RS                                     & 511~                                                                    & ~151 & 6.1        & 43,071~                                                      & 164~                                                                           & 196~                                                           & 93.9      & ~665,236                                                  \\ 
\hline
CS                                     & 27~                                                                     & 1~   & ~0.1       & ~2                                                           & 26~                                                                            & 0~                                                             & 100~      & ~467,425                                                  \\ 
\hline
MS                                     & ~232                                                                    & 47~  & 5.1        & ~6,987                                                       & ~54                                                                            & ~131                                                           & ~94.9     & 132,010~                                                  \\ 
\hline
\rowcolor[rgb]{0.867,1,0.867} CS(or)MS & ~259                                                                    & ~48  & 1.2        & 6,987~                                                       & ~80                                                                            & 131~                                                           & ~98.8     & ~599,435                                                  \\ 
\hline
\multicolumn{9}{|c|}{Group 3}                                                                                                                                                                                                                                                                                                                                                                                                 \\ 
\hline
RS                                     & 534                                                                     & 139  & 6.3        & 42,984                                                       & 163                                                                            & 226                                                            & 93.7      & 648,942                                                   \\ 
\hline
CS                                     & 32                                                                      & 3    & 0.1        & 217                                                          & 27                                                                             & 1                                                              & 99.9      & 462,836                                                   \\ 
\hline
MS                                     & 248                                                                     & 40   & 4.5        & 5,511                                                        & 54                                                                             & 153                                                            & 95.5      & 118,403                                                   \\ 
\hline
\rowcolor[rgb]{0.867,1,0.867} CS(or)MS & 280                                                                     & 43   & 0.9        & 5,728                                                        & 81                                                                             & 154                                                            & 99.1      & 581,239                                                   \\ 
\hline
\multicolumn{9}{|c|}{Group 4 (Collected 9 months after)}                                                                                                                                                                                                                                                                                                                                                                      \\ 
\hline
RS                                     & 1,177                                                                   & 146  & 3.3        & 25,803                                                       & 196                                                                            & 838                                                            & 96.7      & 758,426                                                   \\ 
\hline
CS                                     & 52                                                                      & 4    & 0.1        & 73                                                           & 39                                                                             & 11                                                             & 99.9      & 451,284                                                   \\ 
\hline
MS                                     & 607                                                                     & 43   & 4.2        & 7,575                                                        & 60                                                                             & 505                                                            & 95.8      & 173,785                                                   \\ 
\hline
\rowcolor[rgb]{0.867,1,0.867} CS(or)MS & 659                                                                     & 47   & 1.3        & 7,648                                                        & 99                                                                             & 516                                                            & 98.7      & 625,069                                                   \\
\hline
\end{tabular}}
\end{table}



\subheading{Bottom-Up Results.} Table~\ref{tb:bottom-upDetection} presents the results of our examination of the bottom-up approach using four combinations across the four groups. The findings are as follows. (1) Connection based on redundant sections: Identify the highest number of resilient fingerprints (between 511-1177) but results in a high FP rate (3-6\%) and a TP rate of approximately 93\%-96\%. This method captures around 650K files (65\%) within four groups based on the presence of redundant sections. (2) Connection based on camouflage sections: Identify fewer resilient fingerprints (26-52) but captured a significant number of files (around 450K or 45\%). This approach has a very low FP rate (0.016\%) and a high TP rate (99.9\%). (3) Connection based on malicious sections: Show a slightly higher number of fingerprints (232-273) but triggers a higher FP rate (4\%-5\%) and a lower TP rate (approximately 95\%). This method captures the lowest number of files, around 100K-175K (10-17.5\%) out of 1 million. (4) Combined approach: Based on observations from both CS and MC, combining them results in the best outcomes. It yields a total of resilient fingerprints (around 280-659) with a low FP rate (around 1\%) and a TP rate of $>$98.7\%. This combination identifies more files (between 563K-625 or 50\%-60\%) out of all 1 million files within each group.

% Table~\ref{tb:bottom-upDetection} presents the results of our examination of the bottom-up approach, where we use four combinations across the four groups. First, we analyze the connection based on redundant sections, which identified the highest number of resilient fingerprints (between 511-1177, across the four groups). However, this approach results in a high FP rate of about 3-6\%, and a TP rate of approximately 93\%-96\%. This method identified around 650K out of 1,061,151 (65\%) of the files within three groups, solely based on the presence of redundant sections across their files.
% Secondly, we explore the connection based on camouflage sections, which identify fewer resilient fingerprints (26-52) but capture a much more significant number of files, around 450K out of 1 million (45\%). This approach has a very low FP rate of around 0.016\% and a high TP rate of about 99.9\%.
% Thirdly, we evaluated the connection based on malicious sections, which seemed slightly better on the surface in terms of the total number of campaigns (232-273). However, it triggers a higher FP rate of around 4\%-5\% and a lower TP rate of approximately 95\%. This method captures the lowest total number of files, only around 100K-175K files out of 1 million (~10-17.5\%).
% Finally, based on our observation from both CS and MC, we combine them in the final approach, which provides the best results in terms of total resilient fingerprints (around 280-659), a low FP rate of around 1\%, and a TP rate of >98.7\%, identifying more files between 563K-625 (approximately 50\%-60\%) of all 1 million files within each group.

\subheading{Comparison with Traditional Fingerprinting.} We compare our best findings from the Top-Down and Bottom-Up approaches (highlighted in green) against two traditional fingerprinting techniques: SHA256 and TLSH. For the Top-Down approach, we select the best combination of IL with either CS or MS, while for the Bottom-Up approach, we choose the best-performing CS or MC combinations. In the case of traditional fingerprinting, we consider cryptographic hashes like SHA256 and fuzzy hashes like TLSH. Among the fuzzy hashes, TLSH stands out for its speed and scalability, making it widely adopted by major anti-malware platforms like VirusTotal, Malware Bazaar, MISP, and STIX~\cite{oliver2013tlsh}. Therefore, we use TLSH as a representative for comparison.

Table~\ref{tb:comparision} compares the effectiveness of different fingerprinting methods. SHA256, a cryptographic-based traditional method, has the lowest accuracy (16\% to 18.4\%) in detecting file similarities across all four groups. TLSH, a fuzzy hash-based method, shows slightly better performance, with accuracy ranging from 17\% to 20.7\%. In contrast, our Top-Down and Bottom-Up approaches, utilizing resilient fingerprinting strategies like Import Lists, camouflage sections, and malicious sections, capture a significantly larger number of malware files. The Top-Down approach achieves 30\% to 41.9\% accuracy, while the Bottom-Up approach performs best, with 53\% to 58\% accuracy. However, our approaches also exhibit low false positive (FP) rates, which traditional fingerprinting methods lack. The Top-Down approach has an FP rate of 2.2\% to 3.9\%, while the Bottom-Up approach maintains an FP rate of around 1\%.



% \usepackage{multirow}


\begin{table}
\centering
\caption{Comparison with Tradition Fingerprinting.}
\label{tb:comparision}
%\vspace{-0.3cm}
\resizebox{3.2in}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{\bf Technique} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}{\bf Group 1} \\1,061,151\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}{\bf Group 2} \\1,061,151\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}{\bf Group 3} \\1,061,151\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}{\bf Group 4}\\1,061,151\end{tabular}}  \\ 
\cline{2-9}
                           & \# of files & Acc.~                                                              & \# of files & Acc.                                                               & \# of files & Acc.                                                               & \# of files & Acc.                                                               \\ 
\hline
SHA256                     & 172,102     & 16.2                                                               & 184,592     & 17.4                                                               & 169,891     & 16.0                                                               & 195,655     & 18.4                                                               \\ 
\hline
TLSH                       & 195,028     & 18.4                                                               & 210,027     & 19.8                                                               & 189,493     & 17.9                                                               & 219,304     & 20.7                                                               \\ 
\hline
Top-Down                   & 339,278     & 31.9                                                               & 324,363     & 30.5                                                               & 330,271     & 31.1                                                               & 436,365     & 41.1                                                               \\ 
\hline
Bottom-Up                  & 563,084     & 53.1                                                               & 599,435     & 56.4                                                               & 581,239     & 54.7                                                               & 625,069     & 58.9                                                               \\
\hline
\end{tabular}}
%\vspace{-0.3cm}
\end{table}

\observ{We propose two novel mechanisms, the Top-Down and Bottom-Up approaches, to enhance malware fingerprinting. These methods consistently perform well across four datasets, successfully identifying 30\% to 58\% of reported suspicious files. This represents a significant improvement, up to tripling the identification rate of traditional fingerprinting mechanisms}

==> arxive_esorics/sections/7_summary_discussion.tex <==
\section{Discussion and Limitations}

\subheading{Top-Down vs. Bottom-Up Approaches.}
After systematically evaluating and addressing Q1 and Q2, we discovered key invariant file components that could enhance traditional malware fingerprinting techniques, including cryptographic and fuzzy hash-based methods. To improve the detection of similar malware files utilizing tactics like import lists, camouflage sections, and malicious sections, we developed two innovative techniques: Top-Down and Bottom-Up.
Both methods showed effectiveness, but they had trade-offs. Bottom-Up had superior detection accuracy but tended to capture partially malicious resilient fingerprints with more files, while Top-Down was better at capturing fully malicious ones. We argue that Top-Down may be preferable for capturing the intent of resilient fingerprints. It starts with common Import libraries and then analyzes camouflage and malicious sections, offering insight into intent. In contrast, Bottom-Up may be less effective at identifying intent but more adept at capturing a larger number of malware files that use camouflage and malicious sections, regardless of their import libraries.

\subheading{False Positive Fingerprints.} Our approach deliberately avoided using predictive models like neural networks, relying instead on statistical heuristics for early-stage triaging of connected malware files. While our methods have a low false positive rate, it exists. For example, the Top-Down approach has a 2-3.9\% false positive rate, while the Bottom-Up approach has an even lower rate of 0.7-1.2\%. It's important to note that not all files within false positive clusters have zero malicious vendor labels; some have been labeled malicious by 1-3 vendors. However, our threshold for considering a file malicious requires a minimum of 4 vendor labels, placing these files in the false positive category. Additionally, some files might be highly malicious, but vendors did not detect them when we collected the dataset. Unfortunately, we were unable to confirm this observation.


\subheading{Evaluation of Good Executables.} Obtaining VirusTotal reports for benign executables from external sources posed significant challenges due to IP and legal concerns rather than technical limitations. Submitting benign Windows executables as suspicious to VirusTotal for metadata generation would raise ethical issues given our focus on Windows PE files. However, our dataset already includes a substantial percentage of benign files (\textit{zero}  malicious flags) sourced from VirusTotal, ranging  25\%-35\% in each group, as shown in Table~\ref{tb:benignLabels}. We consider this proportion satisfactory for our research objectives.


\subheading{Packing and Generating Reports Overhead.} Notably, in Figure 1, we emphasize that the VirusTotal platform includes packing type details (e.g., UPX) within the metadata parameters. It's important to note that VirusTotal routinely unpacks these samples before generating metadata. This deliberate omission from our discussion is rooted in the scope of our work. In terms of generation overhead, our study leveraged VirusTotal for metadata generation. Every minute, they supplied metadata for approximately 1,500 received files. However, we selectively utilized detailed metadata, focussing on quick static analysis of sections and import lists as full entities. Typically, these processes demand minimal time, often measured in seconds.


\subheading{Limitations and Future Directions.} Our work has two main limitations. Firstly, while our approach employs more flexible fingerprinting mechanisms to analyze file-invariant parts, it still relies on the hash of these parts as a conservative measure. However, an adaptive attacker could potentially slightly alter these parts, requiring the use of similarity techniques like cosine similarity with an appropriate threshold instead of content hashing. Secondly, our Top-Down approach heavily relies on the import libraries' list of functionalities and content hash for clustering. However, a small percentage of reports collected from VirusTotal lack this content, possibly due to obfuscated import libraries. To address this, we could use API deobfuscation models such as~\cite{cheng2021obfuscation} to rebuild the import libraries list before calculating their content hash, mitigating this limitation.




==> arxive_esorics/sections/8_relatedwork.tex <==
\section{Related Work}

The concept of ``malware fingerprinting'' includes two distinct approaches. The first involves using a defense mechanism to calculate a hash value from suspicious files and sharing it publicly to identify similar files, which is our current focus. The second approach involves observing malware behavior during execution to detect its presence. Additionally, there is an evasion mechanism where malware tries to detect signs of analysis environments or debuggers, as detailed in a study by Afianian et al.~\cite{afianian2019malware}.

%The concept of ``malware fingerprinting'' encompasses two distinct approaches. Firstly, it involves utilizing a defense mechanism that calculates a hash value from suspicious files and shares it publicly to identify similar files at an early stage, which is the focus of our current work. Alternatively, it may entail observing the behavior of malware during execution to detect its presence. The second approach involves an evasion mechanism whereby malware attempts to detect signs of analysis environments or debuggers, as detailed in a study by Afianian et al.~\cite{afianian2019malware}.\\

\subheading{Traditional Fingerprinting.} The use of stream hashing has become a vital technique in malware and threat intelligence. It serves as the first line of defense against cyber threats and is widely used and shared among security teams as checksums or unique identifiers for initial triage. Popular platforms  used for this purpose include VirusTotal, MalwareBazaar, MISP, and STIX~\cite{tlsh}. Security analysts use these identifiers (hashes) as labels and share them with others to identify malware.
Two mechanisms are used to generate these identifiers: cryptographic-based hash and fuzzy-based hash. Cryptographic-based hash relies on cryptographic diffusion, which aims to conceal the relationship between the original entity and the hash, making it a one-way function~\cite{goldmaxMS}. However, even minor changes in the original entity result in a completely different hash. Examples of cryptographic-based hashes include MD5, SHA-1, and SHA256.


To address the limitations of cryptographic-based hash fingerprinting, a more flexible approach called fuzzy hashing is utilized. Fuzzy hashes, like Nilsimsa, TLSH, SSDEEP, or SDHASH, are tolerant of minor changes between files and can capture some malware evasion methods. Among these, TLSH is widely adopted due to its speed and scalability. However, our findings demonstrate that while fuzzy hashes perform better than cryptographic hashes, their effectiveness is still relatively low ($<$20\%) at the file level. This underscores the necessity for more adaptable fingerprinting methods to accurately identify diverse file groups.


\subheading{Dynamic Fingerprinting.} Another work stream focuses on fingerprinting malware based on its execution behavior. Studies by Willems et al.~\cite{willems2007toward} and Rossow et al.~\cite{rossow2011sandnet} found that executing malware for a short period accurately identifies its fingerprint and malicious intent. Kilgallon et al.~\cite{kilgallon2017improving} proposed a systematic mechanism for predicting the time required for sufficient malicious behavior. Küchler et al.
~\cite{kuchler2021does} conducted a study on malware behavior in sandboxes and developed a machine learning-based detection method. They find that multiple sandbox runs may be necessary for reliable behavior fingerprinting. However, this approach may not be suitable for the initial triaging of thousands of suspicious files.

% Another relevant stream of work focuses on fingerprinting malware based on its execution behavior. Willems et al.~\cite{willems2007toward} found that executing malware for two minutes accurately identified its fingerprint and behavior. Rossow et al.~\cite{rossow2011sandnet} executed a large corpus of malware files for an hour and found that five minutes was a reasonable time for malware to exhibit its malicious intent, allowing for the identification of its fingerprint. Kilgallon et al.~\cite{kilgallon2017improving} proposed a systematic mechanism for predicting the time required for a sample to exhibit enough malicious behavior for the heuristics of the cuckoo sandbox, allowing for the assignment of a score of maliciousness.
% Recently, Küchler et al.~\cite{kuchler2021does}  conducted a systematic study of the time-based evolution of malware behavior in sandboxes, and developed a machine learning-based malware detection method based on the insights gained from this study. Some of their takeaways were that one sandbox might not be sufficient to identify malware behavior and that 2-3 sandbox runs might be necessary to obtain reliable behavior fingerprinting.
% While this stream of work may have reasonable efficacy as the malware is in action, it may not be suitable for the first stage triaging where thousands of suspicious files are reported and require an easy early-stage filtering mechanism.

\subheading{Systematic Studies.} Several recent large-scale studies have examined different aspects of malware evasion. Barr-Smith et al.~\cite{barr2021survivalism} focused on the Living off the land technique and found detection gaps among the top 10 AntiVirus products. Alrawi et al.~\cite{alrawi2021circle} compared the lifecycle of IoT malware with traditional desktop-targeting malware and highlighted differences in infection vectors and command and control communication. Cozzi et al.~\cite{cozzi2018understanding} studied Linux-targeting malware and observed similar tactics to Windows malware. Duan~\cite{duan2018things} conducted a study on Android packers using whole-system emulation. Wong et al.~\cite{yong2021inside} proposed a malware analysis taxonomy and recommended guidelines for developers. 
However, \textit{to the best of our knowledge, no large-scale systematic study has explored the limitations of traditional malware fingerprinting for detection and the need for more adaptable mechanisms to identify mutated files with common intent, which motivated the current work.}

% In recent times, several large-scale studies have been carried out on the orthogonal path to comprehend the dynamics and tactics of malware evasion.  For instance, Barr-Smith et al.~\cite{barr2021survivalism} delved into the Living off the land  technique, which uses binaries already present in the system to perform malware actions, and detected gaps in detection among the top 10 AntiVirus products. Alrawi et al.~\cite{alrawi2021circle} examined the lifecycle of IoT malware, compared it with traditional desktop-targeting malware, and identified key differences in infection vectors and command and control communication. Similarly, Cozzi et al.~\cite{cozzi2018understanding} conducted a systematic study of malware that targets Linux instead of Windows, where attackers employed similar tactics as in Windows, such as obfuscating API calls in the ELF loaders and libraries. Duan~\cite{duan2018things} conducted a large-scale systematic study of Android packers through whole-system emulation. Wong et al.~\cite{yong2021inside} carried out a systematic user study and proposed a taxonomy of malware analysis, identified five common analysis workflows and the challenges they faced, and finally recommended guidelines for the developers of malware analysis tools.

% To the best of our knowledge, no large-scale systematic study has investigated the limitations of traditional malware fingerprinting for detection and explored more adaptable mechanisms that would enable security analysts to identify more mutated files that belong to the same intent campaign. This gap was the primary motivation for our work.

==> arxive_esorics/sections/9_conclusion.tex <==
\section{Conclusion}
This paper addresses the gap in understanding of how malware authors bypass traditional file-level fingerprinting and proposes novel approaches to enhance malware fingerprinting. We presented a large-scale empirical analysis of Windows PE files from VirusTotal and identified both invariant and evasive variant parts within these files. The two proposed approaches, Top-Down and Bottom-Up, aim to cluster files using resilient fingerprinting strategies based on similarities in their Import Libraries and sections to improve detection of similar malware files with variations. The results indicate a potential improvement of more than 50\% in detecting similar malware files with variants within a large dataset compared to traditional fingerprinting methods. These findings highlight the importance of updating malware file-level detection fingerprinting methods to stay ahead of evolving evasion mechanisms employed by malware authors. 
